Grammar Prompting for Domain-Specific Language Generation with Large Language Models

Large language models (LLMs) can learn to perform a wide range of natural language tasks from just a handful of in-context examples. However, for generating strings from highly structured languages (e.g., semantic parsing to complex domain-specific languages), it is challenging for the LLM to generalize from just a few exemplars. We propose \emph{grammar prompting}, a simple approach to enable LLMs to use external knowledge and domain-specific constraints, expressed through a grammar in Backus--Naur Form (BNF), during in-context learning. Grammar prompting augments each demonstration example with a specialized grammar that is minimally sufficient for generating the particular output example, where the specialized grammar is a subset of the full DSL grammar. For inference, the LLM first predicts a BNF grammar given a test input, and then generates the output according to the rules of the grammar. Experiments demonstrate that grammar prompting can enable LLMs to perform competitively on a diverse set of DSL generation tasks, including semantic parsing (SMCalFlow, Overnight, GeoQuery), PDDL planning, and SMILES-based molecule generation.

==> figures/acrylates.tex <==
\chemfig[atom style={scale=0.45}]{-[:90](=[:150])-[:30](=[:90]O)-[:330]O-[:30]-[:330]-[:30]O-[:330]%
=^[:270]-[:330]=^[:30]-[:90]=^[:150](-[:210])}


==> figures/blocks_goal.tex <==
\begin{tikzpicture}[scale=0.5]
  %
  \draw (0,0) rectangle (1,1);
  \node[transform shape=false] at (0.5,0.5) {A};
  
  %
  \draw (0,1) rectangle (1,2);
  \node[transform shape=false] at (0.5,1.5) {C};

  %
  \draw (0,2) rectangle (1,3);
  \node[transform shape=false] at (0.5,2.5) {B};

  %
  \draw (1.2,0) rectangle (2.2,1);
  \node[transform shape=false] at (1.7,0.5) {D};
\end{tikzpicture}


==> figures/blocks_init.tex <==
\begin{tikzpicture}[scale=0.45]
  %
  \draw (0,0) rectangle (1,1);
  \node at (0.5,0.5) {A};
  
  %
  \draw (0,1) rectangle (1,2);
  \node at (0.5,1.5) {B};

  %
  \draw (1.2,0) rectangle (2.2,1);
  \node at (1.7,0.5) {C};

  %
  \draw (2.4,0) rectangle (3.4,1);
  \node at (2.9,0.5) {D};
\end{tikzpicture}
